FogROS2-FT: Fault Tolerant Cloud Robotics

Cloud robotics enables robots to offload complex computational tasks to cloud servers for performance and ease of management. However, cloud compute can be costly, cloud services can suffer occasional downtime, and connectivity between the robot and cloud can be prone to variations in network Quality-of-Service (QoS). We present FogROS2-FT (Fault Tolerant) to mitigate these issues by introducing a multi-cloud extension that automatically replicates independent stateless robotic services, routes requests to these replicas, and directs the first response back. With replication, robots can still benefit from cloud computations even when a cloud service provider is down or there is low QoS. Additionally, many cloud computing providers offer low-cost spot computing instances that may shutdown unpredictably. Normally, these low-cost instances would be inappropriate for cloud robotics, but the fault tolerance nature of FogROS2-FT allows them to be used reliably. We demonstrate FogROS2-FT fault tolerance capabilities in 3 cloud-robotics scenarios in simulation (visual object detection, semantic segmentation, motion planning) and 1 physical robot experiment (scan-pick-and-place). Running on the same hardware specification, FogROS2-FT achieves motion planning with up to 2.2x cost reduction and up to a 5.53x reduction on 99 Percentile (P99) long-tail latency. FogROS2-FT reduces the P99 long-tail latency of object detection and semantic segmentation by 2.0x and 2.1x, respectively, under network slowdown and resource contention.

==> acks.tex <==
% \section*{Acknowledgements}

\section*{Acknowledgement}
This research was performed at the AUTOLAB at UC Berkeley in affiliation with the Berkeley AI Research (BAIR) Lab. The authors were supported in part by donations from  Bosch, Toyota Research Institute, Google, Siemens, and Autodesk and by equipment grants from PhotoNeo, NVidia, and Intuitive Surgical. The research is also supported by C3.ai Digital Transformation Institute for AI resilience. 


% This research was performed at the AUTOLab at UC Berkeley in affiliation with the Berkeley AI Research (BAIR) Lab, the CITRIS ``People and Robots'' (CPAR) Initiative, the Real-Time Intelligent Secure Execution (RISE) Lab, and by the NSF/VMware Partnership on Edge Computing Data Infrastructure (ECDI) Secure Fog Robotics Project Award 1838833. This research was supported in part by Bosch. 
% We thank our colleagues for helpful discussions and testing.

==> chapters/introduction_v0.tex <==
% \eric{intro+related work 2 pages, design 2 pages, eval 2 pages, conclusion+references 2 pages}
% \eric{alternative names: 
% FogROS2-SPOT: Server-based Parallel Operations for fault Tolerance; 
% FogROS2-CRAFT: Cloud Robotics With Cost-Reduced And Fault-Tolerant Replicated Servers; 
% CARE - Cloud fAult-tolerant Replicated sErvers; or just FogROS2-FT }
\section{Introduction}
% \eric{cloud robotics reduce cost, enhance performance, ease of management by orchestrating all the computation to a centralized server}
Cloud robotics enables robots to access shared resources and services on-demand with boosted performance and simplified management. More sophisticated algorithms, such as \eric{}, can be deployed on robots without the need for powerful on-board hardware, such as GPU, TPU, and high performance CPU.
In previous research, we developed FogROS2, which enables unmodified robotics code in Robot Operating System 2 (ROS2) to offload heavy computing modules to on-demand cloud hardware resources and accelerators. 
In this work, we introduce a fault-tolerant extension to FogROS2~\cite{ichnowski2022fogros} that is more cost-efficient than previous systems while simultaneously having more robust performance. \jeff{Let's figure out if we want to motivate primarily as a fault-tolerant system or a cost-efficiency system. I propose motivating primarily around fault tolerance will be more impactful (it's probably the main objection we've seen in prior reviewer's comments), but then adding `we also get cost savings' is a surprising bonus} \trinity{agreed; In this work, we introduce a fault-tolerant extension to FogROS2~\cite{ichnowski2022fogros} that is more robust to potential disruptions and has the added benefit of cost-efficiency.}

% \eric{However, cloud introduces factor of unreliablitiy. Traditionally when a robot's compute is broken, but regional network congestions and downtime may affect all the robots, thus affecting the entire operation. The breakdown of the computational service leads to as little as latency disturbances to safety-critical. }
 
% However, the shift towards cloud computing raises issues for the reliability of long-running, safety-critical tasks. In traditional setups, a failure in a single robot's computing resources has limited, localized effects. In contrast, cloud computing introduces vulnerabilities not present in onboard computing systems, such as regional network congestion and server outages, which can impact the operations of an entire fleet of robots. This vulnerability may lead to misconceptions that  cloud robotics are not suitable for safety-critical and long-duration operations.


% \eric{Fault tolerance becomes a requirement for cloud robotics to ensure the reliable task of every request.  however, there are a few factors that makes this challenging. (1) costly by replication, (2) hard to deploy, require engineering}
Fault tolerance allows cloud-robotics tasks to continue operating effectively despite failures in cloud or network components, ensuring the necessary reliability for processing every request. \jeff{`Every' is over promising. I suggest that we should shift the focus (and introduce the robotics audience to) the notion of uptime/downtime ratios and even perhaps SLAs (e.g., \url{https://aws.amazon.com/compute/sla/}).} \eric{help think about (equation), oh cloud would be down}
Achieving such resilience, however, presents notable challenges: as it typically demands an in-depth understanding of the algorithm and specific adaptations for fault resistance, and it involves complex deployment and management processes that require extensive engineering expertise. 
Thus, there can be a misconception that cloud robotics are not suitable for long duration operations. 
%In this work, we recognize the fact that a failure in non-cloud robot systems is fatal; in contrast, 
However, cloud computing can provide redundancy and thus be more reliable, even though cloud networks are more prone to \jeff{Let's avoid using `prone to', we don't want to give the reader the impression that the cloud is worse than it is---that might leave them with the impression that they should avoid the cloud.} regional network congestion and server outages \jeff{Let's see if we can find historical data on actual outages/uptime rates.}. \algname provides fault tolerance for heterogeneous stateless robotic algorithms without requiring ROS2 application modifications. It simultaneously dispatches requests to identical services deployed in multiple cloud data centers and uses the first response received from the replicated services. This model \eric{significantly increases the probability of getting a} timely \jeff{`timely` sounds like its overpromsing too. e.g., all services are slow means it will be slow (but still faster than the slowest). Is there another wording?} responses as long as at least one replica and network remains operational.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/use_case.png}
    \caption{\textbf{\algname} Cloud robotics applications such as grasp planning, are typically deployed on a single typical cloud server, which subjects to single point of failure. Without any ROS2 application modifications, \algname is more cost-efficient than conventional cloud servers launched with FogROS2, and can be fault tolerant to individual server termination or slowdown. }
    \label{fig:intro:use_case}
\end{figure}


% \eric{specifically use replication to for fault tolerance, which further leads to following challenges: (1) ROS2 programming model does not consider replication (2) replicating and dispatching requests across replicas become computationally expensive, }
 
We design a routing network that connects a robot with a scalable number of replicated services, and filters replicated response once the request is handled. The routing network allows resilient and location independent connectivity that persists even if started on a different machine. We propose a compute-efficient threading model for asynchronously processing the requests, and an efficient memory model that eliminates copying memory operation when replicating the message.  \eric{need to sync with the design section}


% \eric{in this work, we takes it to an extreme by building a fault tolerance layer on top of cloud \textit{spot} instances. which it can preemptied at any time. this is challenging for latency critical tasks, creating a new instance can take up to 20 minutes (3) resiliently manage and route all the replicas across multiple cloud and regions.} 
\algname uses {Spot} Virtual Machines (VM), a cost-saving purchasing option offered by major cloud service providers\footnote{In Google Cloud Platform (GCP) and Microsoft Azure, these are called \emph{Spot Virtual Machines}. In Amazon Web Services, these are called \emph{Spot Instances}. } that are up to a 90\,\% discount off the standard on-demand pricing, because they can be \emph{terminated}\footnote{\emph{Interrupted},  \emph{terminated} and \emph{preempted} can be used interchangeably} \emph{unpredictably}. Earlier studies~\cite{10.1145/3458336.3465301} show a bioinformatics task with 24 spot virtual machines on Google Cloud Platform experiences a preemption every 36 minutes on average. 
%Re-creating and initiating a new instance with FogROS2 can take up to 20 minutes \jeff{$\leftarrow$ seems like extraneous information in this context. move elsewhere.}. 
Spot Virtual Machines (VMs) are usually used for non time-sensitive jobs that can be interrupted without significant consequences. 
With the fault tolerance layer in \algname, even time-sensitive robotics tasks can be executed on those cost-effective servers with per-request fault tolerant guarantee, enjoying the benefits of lower expenses without suffering from the drawbacks of unplanned server termination. \algname resiliently manages a pool of spot VMs across multiple cloud and regions, and recreate new spot VM if a replica gets terminated. 

% \eric{\algname achieves 2x fault tolerance with 30\% cost reduction compared to running standard cloud machines on XXX task. }
We evaluate \algname on 4 cloud robotics applications, visual object detection with YOLOv8~\cite{redmon2015you}, semantic segmentation with Segment Anything~\cite{kirillov2023segment}, motion planning with Motion Planning Templates (MPT)~\cite{ichnowski2019mpt}, and a physical Pick-and-Place task with a UR10e. We show that \algname is able to reduce deployment cost of X times, X times compared to standard non-fault-tolerant environment, and x times, X times, X times compared to standard fault-tolerant (again somewhere here emphasize that reduce long tail, won't really notice the benefit of FT on a fast run, but will notice it on a slow run)


This paper makes four contributions: (1) An open-source fault tolerant extension to FogROS2 that enables robots to leverage replicated cloud resources and stay available as long as one of the replica and network is available (2) Cost-effective and reliable Cloud Robotics deployment on spot VMs (3) Cost, fault tolerance and latency data from an experimental evaluation of \algname on 4 cloud robotics applications (4) Physical fault tolerance and cost evaluation with pick-and-place demonstration.

==> chapters/related_work_v0.tex <==
\section{Related Work}

% \eric{skeleton: three paragraphs (1) cloud robotics, (2) latency (vpn(fogros2), fogros-LS paper, sgc) (3) Cloud pricing: Sky, spot instance papers, fogros sky} 
\trinity{second draft - 03/05 2:45pm}

% 1. cloud robotics
\textbf{Cloud and Fog Robotics}.
The use of cloud computing resources for robots, conceptualized as cloud robotics \cite{kehoe2015survey}, has become increasingly relevant
as large models (e.g. NeRF \cite{wang2021nerf} and SAM \cite{kirillov2023segment} for visual perception) and other computationally demanding algorithms (e.g. MPPI for path planning) are integrated in robotic applications.
\trinity{maybe include autonomous vehicle from Prof. Stoica \citet{schafhalter2023cloudav}} \eric{yes peter's paper is definitely relevant}
Following the Fog Computing paradigm \cite{bonomi2012fog}, Fog Robotics \cite{gudi2017fog} utilizes edge resources to improve performance, enabling the viability cloud computing for a multitude of robotics applications, including grasp planning~\cite{tanwani2019fog}, motion planning~\cite{ichnowski2020fog}, visual servoing~\cite{tian2019fog}, and human-robot interaction~\cite{gudi2018fog}.
In the FogROS2 series of work, we address several concerns of using cloud compute for robotics.

% 2. latency, fogros-ls, sgc
\textbf{FogROS2 and Extensions}.
FogROS2 \cite{chen2021fogros} is a cloud robotics framework officially supported by ROS2 \cite{macenski2022robot}.
In terms of network architecture, FogROS2 focused on optimizing for a single cloud and robot using a Virtual Private Network (VPN). Extensions of this work has addressed
% multi-robot and multi-cloud capabilities.
the questions of connectivity, latency, and cost.
\sgc (Secure and Global Connectivity) \cite{chen2023fogros} connects distributed ROS2 nodes in a peer-to-peer network, enabling secure communication between robots.
% Additionally, we address latency concerns in
FogROS2-LS (Latency Sensitive) \cite{chen2024fogrosls} adopts \emph{anycast} \cite{ballani2005anycast} communication so that a robot can flexibly switch to using one of many servers to meet latency requirements.
% FogROS2-Pilot \cite{chen2024sky} is able to select a cloud machine across multiple clouds (Amazon Web Services, Google Cloud Platform, Microsoft Azure) by extending SkyPilot \cite{yang2023skypilot}, an "intercloud broker." 
% In FogROS2-Pilot \cite{chen2024sky}, we follow the philosophy of Sky Computing \cite{chasins2022sky}, where cloud compute across providers are treated as one commodity.
% By querying SkyPilot \cite{yang2023skypilot}, an intercloud broker,
% FogROS2-Pilot selects a cloud machine across multiple clouds\footnote{The supported clouds are Amazon Web Services (AWS), Google Cloud Platform (GCP), and Microsoft Azure. \trinity{are there others?}} that meets user-specified time and cost per request.
FogROS2-Pilot \cite{chen2024sky} alleviates roboticists from having to navigate hundreds of available cloud machine by automatically selecting a that meets user-specified time and cost per request.


% 3. cloud pricing, spot instance, fogros sky
\textbf{Spot VMs}.
FogROS2-Pilot focuses on selecting a cloud machine with the ideal hardware specifications, but cloud providers offer a wide variety of pricing options that differ beyond hardware.
% Cloud providers offer a wide variety of pricing options \cite{wu2019cloudpricing} based on hardware specifications and availability.
Spot VMs\footnote{In Google Cloud Platform (GCP) and Microsoft Azure, these are called \emph{Spot Virtual Machines}. In Amazon Web Services, these are called \emph{Spot Instances}. More generally, they are also known as \emph{preemptible} or \emph{transient} machines.}
are one such cost-saving purchasing option offered by major cloud service providers that are up to a 90\,\% discount off the standard on-demand pricing, because they can be \emph{preempted}\footnote{\emph{Preempted},  \emph{terminated} and \emph{interrupted} can be used interchangeably.} \emph{unpredictably} \cite{amazon2021spot}. 
The rates of preemption are highly variable across regions and instance types, from 3\% to over 20\% chance of preemption per day.
The prices are also variable, and can even fluctuate over the course of a single day.
Extensive research has been done to predict spot pricing using statistical models \cite{javadi2011spotpricemodeling} \cite{singh2015spotpricepredict} and learning methods \cite{baughman2018spotpricelstm} \cite{khandelwal2020spotpricerrf}.
Due to their unreliable nature and lack of guarantees, spot VMs were not considered as part of the machine selection in FogROS2-Pilot.
From a user perspective, there is an economic trade-off of the reduced price of spot VMs and having to build an infrastructure handling shutdowns and restarts \cite{li2016spotpricereview}.
% \cite{lee2023spoteconomics} \cite{george2019awsspot}.

Fortunately, a fault tolerant system is naturally compatible with spot VMs. The core components of a fault tolerant system are \emph{redundancy}, duplicated machines ensuring operation in case of a failure on one system, and \emph{failover}, dynamically switching to one of the replica machines upon failure of one machine.
\citet{voorsluys2012reliablespot}, \citet{poola2016spot}, and \citet{pergentino2019mults} among others have demonstrated that spot instances can be used as a cost-efficient, fault-tolerant setup.
Spot instances have been used successfully for multiple applications including web services \cite{alieldin2019spotweb}, deep learning \cite{lee2017deepspotcloud}, but spot usage has not yet been explored for robotics.

\eric{merge fogros2(sky) with spot instances; include related work for fault tolerance}

% \textbf{Fault Tolerance}
% ... \citet{hasan2018ftsurvey} \trinity{there are different ``levels" of fault tolerance; proactive vs reactive measures, etc. should we go into this?}
% \eric{a high level overview of existing methods is fine. We say: we leverage the uniqueness of the cloud (if there is no existing work on that).}


\section{System Assumptions and Features}

\subsection{System Assumptions}
In this work, we assume the applications adhere to ROS2 request-response communication model. The application can be partitioned as a client that sends sensor data as requests and await control instructions as response, and service implemented as ROS2 services that can be offloaded to the cloud. 
%The robot needs to have a stable connection to at least one of the cloud machines. The application needs to computational capacity of the cloud needs to handle the request requirement to receive timely response. 
The services need to be stateless to achieve fault tolerance without application awareness, or applications needs to use well-defined interfaces from \algname to make the states consistent.
% It cannot protect from application software bugs.  % omit - goldberg
% \eric{assume each svm is independent and failures are not correlated}

\subsection{\algname Failure Qualification}
% \ken{qualify as P(failure) = 1-P(fail1)*P(fail2)}
Multiple cloud servers can provide fault tolerance independent against region or server-specific compute or network failures. 
% \trinity{from Christian J: ``Maybe important to discuss: which types of failures are targeted in detail, and can we quantify the likelihood of these failures (eg SLAs)? The paper is stronger if we don't need the cost aspect to justify its usefulness"}
We assume the robot has a persistent and stable connection to at least one of the cloud servers. 
Since \algname can launch cloud servers across different regions and cloud service providers, the probability of simultaneous failures from independent cloud service providers or regions is independent.

% REFRAME MATH SECTION
% % We qualify the failure of \algname as following:  The Spot VM can be terminated unpredictably. 
% % We define the failure as following: 
% The probability of a server failing can be estimated as:
% \[
% P(\text{Failure of VM}_i) = 1-\frac{\text{uptime of VM}_i}{\text{uptime}_i + \text{recovery time}_i}
% \]

% % \ken{VM to Spot VM} \eric{actually here we can be more general, as spot VM's failure is just a type of VM failure}
% % As a result, the failure of \algname can be qualified as 
% As a result, the probability of a system failure with N replicated VMs is:
% \[
% % P(\text{Failure}) = 1 - \prod_{i \in \Theta} P(\text{Failure of VM}_i)
% P(\text{Failure}) = 1 - \prod_{i \in N} P(\text{Failure of VM}_i)
% \]
% % where $\Theta$ is the set for all the VMs. \eric{this formulation assumes the number of replica is constant}
% NEWLY REFRAMED MATH SECTION
The probability of one VM failing can be estimated as
\[
P_{\text{VM}_i}(\text{failure}) = 1-\frac{\text{uptime}_{\text{VM}_i}}{\text{uptime}_{\text{VM}_i} + \text{recovery time}_{\text{VM}_i}}
\]
and the probability of a system failure with $N$ replicas is
\[
P_{\text{system}}(\text{failure}) = \prod_{i \in N} P_{\text{VM}_i}(\text{failure})
\]
% Given the desired maximum failure rate for the system $P_{\text{system}}(\text{failure}) = \epsilon$ and assuming the preemption rate for spot VMs $P_{\text{VM}_i}(\text{failure}) = \delta$, we can calculate the required $N$ number of replicas as
Given the desired maximum failure rate for the system and estimating the failure rate for all VMs used, we can calculate the required $N$ number of VM replicas as
   \[  N = \left\lceil \frac{\log{P_{\text{VM}}(\text{failure})}}{\log{P_{\text{system}}(\text{failure})}} \right\rceil \]

To reduce the probability of failure, one can either increase the number of replicas, or use a combination of spot and on-demand instances. 
Assuming a spot VM is preempted every 15 hours on average and re-creating and initiating a new instance with FogROS2 can take up to 20-minute downtime, the probability of simultaneous preemptions with two spot VMs is less than 0.05\%. \trinity{suggestion: calculate using the typically provided spot rates of preemption chance per day (from 5\% to $>$20\%). Using a 20\% machine would still result in $<$0.05\% failure}
% Probability is lowered if more replicas are used. % move to earlier - goldberg 
% One can also mix the cloud server with spot VM to further reduce the failure rate. % ?? - goldberg

\subsection{New Features}

\algname is distinguished from previous work with the following features: 

\begin{enumerate}
    \item \textbf{Fault Tolerance}. \algname features \textit{per-request} fault tolerance, ensuring requests can be fulfilled as long as at least one replica and network remains operational.
    \item \textbf{Cost-Effectiveness}.  \algname can provide significantly lower cost by using spot VMs
    \item \textbf{Algorithm Agnostic Fault Tolerance}. \algname operates independently of the specific algorithms used in applications as long as it is stateless 
    \item \textbf{Failure Cause Agnostic}. \algname does not need to be tailored to specific failure scenarios, and remains functional as long as at least one service is available and connected.
    \item \textbf{Multi-Cloud, Multi-Region Fault Tolerance}. Since the failure may occur to a specific region or cloud provider, \algname, as part of the Sky Computing paradigm, offers a unified interface for interacting with various cloud service providers and leverages cloud computing resources across different clouds simultaneously. 
    \item \textbf{Scalability}. \algname allows robots to launch a scalable number of machines to set the probability that all the replica service deployments are not available. 
    \item \textbf{Adaptive and Resilient Recovery}. \algname automatically recovers from service interruptions, preserving the intended level of fault tolerance automatically.
    % \item \textbf{Seamless ROS2 Application Integration:} With \algname, there's no need for modifications to existing ROS2 applications; they can be offloaded to the cloud and will function as though all ROS2 components were located on a single machine. 
\end{enumerate}

==> chapters/related_work_v1.tex <==
\section{Related Work}

% \eric{skeleton: three paragraphs (1) cloud robotics, (2) latency (vpn(fogros2), fogros-LS paper, sgc) (3) Cloud pricing: Sky, spot instance papers, fogros sky} 
% \trinity{second draft - 03/05 2:45pm}

% 1. cloud robotics
\paragraph*{Cloud and Fog Robotics}
The use of cloud computing resources for robots, conceptualized as cloud robotics~\cite{kehoe2015survey}, has become increasingly relevant
as large models (e.g., NeRF~\cite{wang2021nerf}, SAM~\cite{kirillov2023segment} and LERF~\cite{Rashid24lifelonglerf} for visual perception) and other computationally demanding algorithms (e.g., MPPI for path planning) are integrated in robotic applications.
Following the Fog Computing paradigm~\cite{bonomi2012fog}, Fog Robotics~\cite{gudi2017fog} utilizes edge resources to improve performance, enabling the viability cloud computing for a multitude of robotics applications, including grasp planning~\cite{tanwani2019fog}, motion planning~\cite{ichnowski2020fog}, visual servoing~\cite{tian2019fog}, and human-robot interaction~\cite{gudi2018fog}.
In the FogROS2 series of work, we address several concerns of using cloud compute for robotics.
FogROS2~\cite{chen2021fogros} is a cloud robotics framework officially supported by ROS2~\cite{macenski2022robot}.
%In terms of network architecture, 
FogROS2 focused on optimizing for a single cloud and robot using a Virtual Private Network (VPN). Extensions of this work has addressed
% multi-robot and multi-cloud capabilities.
the questions of connectivity, latency, and cost.
\sgc (Secure and Global Connectivity)~\cite{chen2023sgc} enables secure communication between distributed ROS2 robot nodes.
% Additionally, we address latency concerns in


% 2. latency, fogros-ls, sgc
\paragraph*{Multi-Cloud Robotics}
FogROS2 is the first multi-cloud robotics that offloads robotics applications to multiple cloud service providers. 
FogROS2-Config~\cite{chen2024fogrosconfig} extend FogROS2 to  navigate available cloud machine selection that meets user-specified time and cost per request.
\algname uses multi-cloud Spot VMs to reduce the cost of the deployment. Spot VMs 
are one such cost-saving purchasing option offered by major cloud service providers that are up to a 90\,\% discount off the standard on-demand pricing, because they can be \emph{preempted}\footnote{\emph{Preempted},  \emph{shut down} and \emph{interrupted} are used interchangeably.} \emph{unpredictably}~\cite{amazon2021spot}. This creates trade-off between the reduced price of spot VMs and having to build an infrastructure handling shutdowns and restarts~\cite{li2016spotpricereview}.
The rates of preemption are highly variable across regions and instance types, from 3\,\% to over 20\,\% chance of preemption per day.
Spot VM prices are also variable, and can fluctuate over the course of a day.
Extensive research has been done to predict spot pricing using statistical models~\cite{javadi2011spotpricemodeling,singh2015spotpricepredict} and learning methods~\cite{baughman2018spotpricelstm,khandelwal2020spotpricerrf}.
Due to their unreliable nature, spot VMs were not considered as part of the machine selection in FogROS2 and FogROS2-Config.

% FogROS2-Config focuses on selecting a cloud machine with the ideal hardware specifications, but cloud providers offer a wide variety of pricing options that differ beyond hardware.
% Cloud providers offer a wide variety of pricing options \cite{wu2019cloudpricing} based on hardware specifications and availability.



% \cite{lee2023spoteconomics} \cite{george2019awsspot}.

\paragraph*{Fault Tolerance for Latency Sensitive Applications} 
% A fault tolerant system is naturally compatible with spot VMs. 
A fault tolerant system is typically based on \emph{redundancy} by duplicated machines ensuring operation in case of a failure on one system, and \emph{failover}, dynamically switching to one of the machines upon failure of one machine.
FogROS2-LS (Latency Sensitive)~\cite{chen2024fogrosls} adopts \emph{anycast}~\cite{ballani2005anycast} communication so that a robot can flexibly connect to using one of many servers, but the system takes time to discover and recover from faults by switching to another server that meets latency requirements.
\citet{schafhalter2023cloudav} improves the responsiveness of autonomous vehicles by performing operations on both vehicle and cloud. 
\citet{wu2018visual} statistically models and detects anomalous time series events.
\citet{voorsluys2012reliablespot,poola2016spot,pergentino2019mults} demonstrate spot instances can be used as a cost-efficient, fault-tolerant setup. However, they focus on the cost optimization on a single operation, while the design of reducing faults of continuous and latency-sensitive robotic operations is understudied. Prior work also designed  applications to fault tolerance environment with spot VMs, such as web services~\cite{alieldin2019spotweb} and deep learning~\cite{lee2017deepspotcloud}. \algname can automatically offload off-the-shelf robotics applications to fault-tolerant multi-cloud environment without the awareness of the robotic application developers.



% \eric{merge fogros2(sky) with spot instances; include related work for fault tolerance}

% \textbf{Fault Tolerance}
% ... \citet{hasan2018ftsurvey} \trinity{there are different ``levels" of fault tolerance; proactive vs reactive measures, etc. should we go into this?}
% \eric{a high level overview of existing methods is fine. We say: we leverage the uniqueness of the cloud (if there is no existing work on that).}


\section{System Assumptions and Features}

\subsection{System Assumptions}
We assume
that all servers, networks, and faults are independent, and that 
% \trinity{added this from Goldberg's notes, maybe reformat/reword this}
the applications adhere to ROS2 service communication model. The application can be partitioned as a client that sends sensor data as requests and await control instructions as response, and service implemented as ROS2 services that can be offloaded to the cloud. 
%The robot needs to have a stable connection to at least one of the cloud machines. The application needs to computational capacity of the cloud needs to handle the request requirement to receive timely response. 
The services need to be stateless to achieve fault tolerance without application awareness, or applications needs to use well-defined interfaces from \algname to make the states consistent.
% It cannot protect from application software bugs.  % omit - goldberg
% \eric{assume each svm is independent and failures are not correlated}

\subsection{\algname Failure Qualification}
% \ken{qualify as P(failure) = 1-P(fail1)*P(fail2)}
Multiple cloud servers can provide fault tolerance to region or server-specific compute or network failures. 
% \trinity{from Christian J: ``Maybe important to discuss: which types of failures are targeted in detail, and can we quantify the likelihood of these failures (eg SLAs)? The paper is stronger if we don't need the cost aspect to justify its usefulness"}
We assume the robot has a persistent and stable connection to at least one of the cloud servers. 
% Since \algname can launch cloud servers across different regions and cloud service providers, the probability of simultaneous failures from independent cloud service providers or regions is independent.
% REFRAME MATH SECTION
% % We qualify the failure of \algname as following:  The Spot VM can be terminated unpredictably. 
% % We define the failure as following: 
% The probability of a server failing can be estimated as:
% \[
% P(\text{Failure of VM}_i) = 1-\frac{\text{uptime of VM}_i}{\text{uptime}_i + \text{recovery time}_i}
% \]

% % \ken{VM to Spot VM} \eric{actually here we can be more general, as spot VM's failure is just a type of VM failure}
% % As a result, the failure of \algname can be qualified as 
% As a result, the probability of a system failure with N replicated VMs is:
% \[
% % P(\text{Failure}) = 1 - \prod_{i \in \Theta} P(\text{Failure of VM}_i)
% P(\text{Failure}) = 1 - \prod_{i \in N} P(\text{Failure of VM}_i)
% \]
% % where $\Theta$ is the set for all the VMs. \eric{this formulation assumes the number of replica is constant}
% NEWLY REFRAMED MATH SECTION
The probability of a VM failing at any moment in time is% \jeff{This is at any moment in time, correct? We should state that explicitly if so. If not, can we clarify?}
\[
P_{\text{VM}_i}(\text{failure}) =
% 1-\frac{\text{uptime}_{\text{VM}_i}}{\text{uptime}_{\text{VM}_i} + \text{recovery time}_{\text{VM}_i}}
\frac{\text{recovery\_time}_{\text{VM}_i}}{\text{uptime}_{\text{VM}_i} + \text{recovery\_time}_{\text{VM}_i}}, % <- punctuate equations when used in sentences
\]
and the probability of a system failure with $N$ spot VMs is
\[
P_{\text{system}}(\text{failure}) = \prod_{i \in N} P_{\text{VM}_i}(\text{failure}).
\]
% Given the desired maximum failure rate for the system $P_{\text{system}}(\text{failure}) = \epsilon$ and assuming the preemption rate for spot VMs $P_{\text{VM}_i}(\text{failure}) = \delta$, we can calculate the required $N$ number of replicas as
Given a desired maximum failure rate for the system and the failure rate for all VMs used, we can calculate the required number of VM replicas as
   \[  N = \left\lceil \frac{\log{P_{\text{VM}}(\text{failure})}}{\log{P_{\text{system}}(\text{failure})}} \right\rceil. \]

To reduce the probability of failure, one can either increase the number of replicas, or use a combination of spot and on-demand instances. 
\jeff{The next sentences should be framed as an example. In particular, we cannot expect the preemption rate to be the same throughout the year, or for years to come.}
A spot VM is preempted every 15 hours on average~\cite{yang2023skypilot} and re-creating and initiating a new instance with FogROS2 can take up to 20-minute downtime~\cite{chen2021fogros}, the probability of simultaneous preemptions with two spot VMs is less than 0.05\,\%. 
%\trinity{suggestion: calculate using the typically provided spot rates of preemption chance per day (from 5\% to $>$20\%). Using a 20\% machine would still result in $<$0.05\% failure}
% 15 hours is from skypilot paper 


% Probability is lowered if more replicas are used. % move to earlier - goldberg 
% One can also mix the cloud server with spot VM to further reduce the failure rate. % ?? - goldberg

\subsection{New Features}

\algname is distinguished from previous work with the following features: \jeff{I'm a little concerned that this mostly reads as 1. FT, 2. other, 3. FT, 4. FT, 5. FT, 6. other, 7. other. Not sure the fix. It could be to just remove ``fault tlerance'' from a few. Or make the list hierarchical. Or just ignore this concern.}

\begin{enumerate}
    \item \textbf{Fault tolerance}. \algname features \textit{per-request} fault tolerance, ensuring requests can be fulfilled as long as at least one replica and network remains operational.
    \item \textbf{Cost-effectiveness}.  \algname can provide significantly lower cost by using spot VMs. \jeff{Can we add `Mixed resource type' to highlight that one can mix on-demand and spot instances, and even different spec instances (e.g., low-spec on-demand for up-time, and high-spec spot for speed)}
    \item \textbf{Algorithm-agnostic fault tolerance}. \algname operates independently of the specific algorithms used in applications as long as it is stateless.
    \item \textbf{Failure cause agnostic}. \algname does not need to be tailored to specific failure, and remains functional as long as at least one service is available and connected.
    \item \textbf{Multi-cloud, multi-region fault tolerance}. Since the failure may occur to a specific region or cloud provider, \algname, as part of the Sky Computing paradigm \jeff{cite?}, offers a unified interface for interacting with various cloud service providers and leverages cloud computing resources across different clouds simultaneously. 
    \item \textbf{Scalability} \algname allows robots to launch a scalable \jeff{be a bit more specific with the `scalable' number here---otherwise this is defining the Scalability feature as being scalable.} number of machines to set the probability that all the replica service deployments are not available. 
    \item \textbf{Adaptive and resilient recovery} \algname automatically recovers from service interruptions, preserving the intended level of fault tolerance automatically.
    % \item \textbf{Seamless ROS2 Application Integration:} With \algname, there's no need for modifications to existing ROS2 applications; they can be offloaded to the cloud and will function as though all ROS2 components were located on a single machine. 
\end{enumerate}


==> tables/exp1results.tex <==
% \begin{table}
%     \centering
%     \footnotesize
%     \begin{tabular}{l l l r r } 
% \toprule
%  & Available & Failure  & Prob. Selecting  & Failure \\ 
% & Machines  & Rate (\%)& Edge(\%) &  Reduction\\
% \midrule
% 1&E-M, E-B    & 26.67 (8/30) & - & 1x, \textbf{2.2x} \\
% 2&E-M, C-W    & 6.67 (2/30)     & 30 (9/30)   &  \textbf{4x}, 1.3x \\
% 3&E-B, C-W     & 10.00 (3/30)    &  6.67 (2/30) & \textbf{5.6x}, 1x\\ 
% 4&E-M, C-E      & 30.00 (9/30)  & 46.67 (14/30) & 1x, \textbf{1.1x} \\ 
% 5&E-B, C-E      & 53.33  (16/30)   &  3.33 (1/30)  &  \textbf{1.1x}, 0.63x \\ 
% 6&E-M, C-W, C-E       &  10.00 (3/30)  & 53.33 (16/30) & 2.7x, 1x, \textbf{3.3x} \\  
% 7&E-B, C-W, C-E       &  6.67 (2/30)  & 0 (0/30)  & \textbf{8.5x}, 1.5x, 5x \\  
% \bottomrule
% \end{tabular}
% \caption{\textbf{Evaluation of \algname in Failure Reduction} \algname selects from available baseline machines and we measure the failure rate (lower the better). \algname matches or surpasses the performance of the best individual machine, reducing the failure rate by up to 8.5 times. By selecting a machine with best latency at a given moment, it can achieve even lower failure rate than up to 1.5 times lower than that of any single machine available. \eric{please help check with the numbers, i did the calculation by hand}}
% \label{tab:eval:exp1:results}
% \vspace{-8pt}
% \end{table}

% \begin{table}
%     \centering
%     \footnotesize
%     \begin{tabular}{l l l l } 
% \toprule
%  Failure & Delay: 20 + 50ms   &  Delay: 20 + 50ms\\ 
%  Rate(\%) & 50\%   Applied     &  100\%  Applied  \\
% \midrule
% Edge1(Delay) &  26.7(8/30)  &  56.7 (17/30)        \\
%     + Edge 2 &  0.0  &  0.0       \\
%     + Cloud(West) &  10.0(3/30)  &  6.7   \\
%     + Cloud(East) &  30.0(9/30)  &  53.3   \\
%     + Cloud(East) + Cloud(West) &  6.7(2/30)   &  10.0   \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Evaluation of \algname in Failure Reduction} \algname selects from available baseline machines and we measure the failure rate (lower the better). \algname matches or surpasses the performance of the best individual machine, reducing the failure rate by up to 8.5 times. By selecting a machine with best latency at a given moment, it can achieve even lower failure rate than up to 1.5 times lower than that of any single machine available.}
% \label{tab:eval:exp1:results}
% \vspace{-8pt}
% \end{table}

\begin{table*}
    \centering
    \setlength{\tabcolsep}{10pt} 
    \renewcommand{\arraystretch}{1.5} % Default value: 1

    \footnotesize
    \begin{tabular}  {l | c | c c c c c c} 
\toprule
 % Failure Rate & Edge 1(Delay)  &  Edge 1(Delay) & Edge 1(Delay) & Edge 1(Delay) \\ 

 Edge 1 (Add Delay) & Edge 1 & Edge 1 & & & \\ 
 Failure Rate (\%)  & Only & + Edge 2     &  + Cloud(W) & + Cloud(E) & + Cloud(W) + Cloud(E)  \\
\hline
 100\% Applied &  56.7\% & 0.0\% & 10.0\% & 30.0\% & \bf{6.7\%}    \\
 % \midrule
    (Failure Reduction) &   & $(\infty)$ & (5.7x) & (1.9x) & \bf{(8.5x)}    \\
\hline
    50\% Applied &  26.7\%  & 0.0\% & \bf{6.7\%} & 53.3\% & 10.0\%  \\
% \midrule
   (Failure Reduction) &   &  ($\infty$) & \bf{(4.0x)} & (0.5x) & (2.7x)  \\
    % + Cloud(East) + Cloud(West) &  6.7(2/30)   &  10.0   \\
\bottomrule
\end{tabular}

\caption{\textbf{When local network was congested, \algname reduced failures:} Upon application of random network delays on Edge \#1, \algname automatically re-route to alternative services, i.e. Edge 2, Cloud(W), Cloud(E).  
Such automatic switching functionality to an alternative, location independent service(s) improves robustness of the system and reduced failure rate (lower the better) of the overall system. 
\algname matches performance of the best individual machine, reducing the failure rate by up to 8.5 times by selecting the best available machine compared to single edge service system under heavy network congestion.
We also showed that \algname enabled flexible yet reliable access to open cloud services via Anycast to reduce failure rate.}
\label{tab:eval:exp1:results}
\vspace{-8pt}
\end{table*}

==> tables/exp1setup.tex <==
\begin{table}
    \centering
    \footnotesize
    \begin{tabular}{ l l l | c c } 
\toprule
 & Candidates & Failure  & Interference  & Interference\\ 
  &          & Rate (\%)& (ms) & Prob. (\%)\\
\midrule
 E-G&Edge (Good)    & 0 (0/30)     & 0     & 0\\
 E-M&Edge (Medium)  & 26.67 (8/30) & $35\pm15$ & 50\\ 
 E-B&Edge (Bad)     & 56.67 (17/30)  & $35\pm15$ & 100\\ 
 C-W&Cloud (West US)     & 10  (3/30)   & -     & -\\ 
 C-E&Cloud (East US)       &  36.67 (10/30)  & -     & -\\ 
\bottomrule
\end{tabular}
\caption{\textbf{Failure Rate and Network Setups of Baseline Machines For Visual Distance Estimation}  The robot controller maintains a direct and stable connection to the Edge server via an Ethernet cable. Interference is introduced with a $35\pm15$ ms network delay, applied at rates of 50\% and 100\% to respectively represent Edge (Medium) and Edge (Bad) conditions. All the robots and edge servers are at California (West US), and the Cloud servers are located at AWS facilities in Oregon (West US) and Ohio (East US). \eric{is 35+-15 the same as 20 + 50? the latter one might be confusing} \marcus{Michael says it's just $50 \pm 0$ ms (no randomness).}
}
\label{tab:eval:exp1:setup}
\vspace{-8pt}
\end{table}

==> tables/time.tex <==

% column: application, experiment time, average uptime, total preemptions 
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{@{}l@{\quad}c@{\quad} c@{\quad}c@{\quad}c@{\quad}c@{\;}c@{\;}c@{}}\toprule
           & Experiment & Preemptions & 1 Response  & 2 Response &  \\
           &  Time (hr) & Experienced & Rate (\%)  & Rate (\%)  \\
         \midrule
        
         YOLO &  25  & 2 & 100 & 75  \\
         SAM  &  25  & 3  & 100  & 75 \\ 
         Dex-Net  &  25  &  3 & 100  & 75 \\ 
         MPT  &  25  & 3  & 100  &75 \\ 
         \bottomrule
    \end{tabular}
    \caption{\textbf{\algname experiment uptime on Cloud Robotics applications} We run all cloud robotics applications with more than 24 hours period and experienced more than 2 preemptions. \algname is able to provide at least one response for all the applications despite the preemptions, and with X \% of receiving responses from multiple servers.\eric{response rate are placeholders}  }
    \label{tab:eval:time}
\end{table}

